RED: Robust Environmental Design

The classification of road signs by autonomous systems, especially those reliant on visual inputs, is highly susceptible to adversarial attacks. Traditional approaches to mitigating such vulnerabilities have focused on enhancing the robustness of classification models. In contrast, this paper adopts a fundamentally different strategy aimed at increasing robustness through the redesign of road signs themselves. We propose an attacker-agnostic learning scheme to automatically design road signs that are robust to a wide array of patch-based attacks. Empirical tests conducted in both digital and physical environments demonstrate that our approach significantly reduces vulnerability to patch attacks, outperforming existing techniques.

==> PhysicalExperimentSetUp.tex <==
\subsection{Physical Experiment Setup}
We selected and physically recreated representative road signs for our experimental evaluation. From the LISA dataset, we chose two speed limit signs, a stop sign, and an arrow sign. From the GTSRB dataset, we selected a stop sign, two speed limit signs, and a truck warning sign. These signs are shown in Figure \ref{fig:lisa_signs}.

\begin{figure}[h]
\centering
\includegraphics[width=0.95\textwidth]{images/figure6.png}
\caption{\todo{This figure will go to appendix}}
\label{fig:different_signs}
\end{figure}


\paragraph{Creating Redesigned Road Signs Dataset}
Creating the dataset involves three steps: training, printing, and photo capture with post-processing. First, we search for robust patterns to identify each road sign background.
We then print the design patterns using a \emph{Sony Picture Station} printer onto 16x18 inch paper boards. The margins are trimmed, leaving the actual road sign, which averages 12x12 inches, as shown in Figure \ref{fig:road_sign}.
After producing the road signs, we photographed them in various real-world settings using a Nikon D7000 camera, held by an individual to mimic actual roadside conditions, as shown in Figure \ref{}.
We collected multiple images of each sign under diverse environmental conditions to ensure comprehensive evaluation. These conditions included different locations for varied backgrounds, various weather conditions such as cloudy and sunny days for visibility assessment, and different times of day, particularly morning and evening, to capture varying natural light levels, as shown in Figure \ref{}.
Post-collection, the images underwent a process to closely mimic the photo conditions used in the LISA and GTSRB datasets. Each image was manually cropped to isolate the road sign from background distractions. The images were then resized to the standard dimensions used in these datasets, specifically 30 by 30 pixels, with the actual road sign dimensions roughly ranging from 3 to 27 pixels in both width and height.

\begin{figure}[h]
\centering
\includegraphics[width=0.95\textwidth]{images/figure3.png}
\caption{\todo{This figure will go to appendix}}
\label{fig:color_transformation}
\end{figure}

\paragraph{Training Pipeline Set Up}
After discussing the evaluation of redesigned road signs, we now describe the method used to train for the robust pattern. As mentioned in section \ref{}, we utilized a differentiable image composition pipeline to search for robust patterns. This process involves generating a bird's-eye view pattern at each iteration for each class. The pattern is then warped onto a road sign mask using a homography matrix and color transformations.
The spatial transformation is straightforward; we warp the robust pattern to fit within the road signs.
For color transformation, to ensure our redesigned road signs are robust against different lighting conditions, we tested several color patches by printing them and taking photos under various times and lighting conditions. Specifically, to accurately learn the color mapping, we used Kelly's 22 most contrasting colors. These colors were printed and photographed under diverse environmental conditions to collect data on color transformations. The 22 color patches were exposed to different times of the day and varying weather conditions, simulating real-world variations and ensuring our model can generalize well across typical and atypical lighting and weather scenarios. The process can be visualized in Figure \ref{}.
After collecting the photos, we classified them into several diverse lighting conditions, varying by weather and time. We then used a three-layer neural network with ReLU activations to model the color transformations. As depicted in Figure \ref{fig:example_label}, the variations in color perception under different lighting conditions highlight the effectiveness of our calibration process.

\subsection{Attack Implementation Details}
\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{images/figure8.png}
\caption{\todo{Need to Update}}
\label{fig:my_label}
\end{figure}

We include various patch shapes, such as circles, triangles, rectangles, and sticker attacks proposed by \ref{multi_sticker_ref}, as shown in Figure \ref{}. We assume the attacker has full access to the classification model \( f \) and the patches.

We propose an attack specifically tailored for patch-based inference:
\todo{Formalize this algorithm}
\begin{enumerate}
    \item Identify patches with \( f(s) = y \) to obtain \( S_c \).
    \item Divide the attack into \( M \) parts.
    \item For each \( m \) in \( M \), attack one patch and remove the successfully attacked patch from \( S_c \).
\end{enumerate}
We used 100 iteration for finding the attack, and the step size is 0.01

==> abstract.tex <==
\section{abstract}
Robust Design


==> attack.tex <==
\section{Attacks}
only very briefly introduce patch 
\todo{Ignore this section. This section need to be rewrite! }
We focus on defending against the physically realizable attack, typically in the form of a patch attack. Let \( x \) be the original input image, and \( x_{\text{adv}} \) the adversarial image obtained after the patch attack. We denote \( \delta \) as the adversarial patch applied to the original image \( x \). The patch attack is defined as follows:

Given an original image \( x \) and an adversarial patch \( \delta \), the adversarial image \( x_{\text{adv}} \) is obtained by adding the patch \( \delta \) to the original image \( x \), element-wise:
\[
x_{\text{adv}} = x + \delta
\]
This equation signifies that for each pixel in the original image \( x \), the corresponding pixel in the adversarial image \( x_{\text{adv}} \) is obtained by adding the corresponding pixel from the patch \( \delta \).

Under the assumption of a per-image attack, every victim image is considered a potential target for the patch attack. Therefore, for each victim image \( x_i \), an adversarial image \( x_{\text{adv}_i} \) is generated by applying the patch \( \delta \) to \( x_i \):
\[
x_{\text{adv}_i} = x_i + \delta
\]
This equation implies that the patch attack is performed individually on each victim image \( x_i \), resulting in an adversarial image \( x_{\text{adv}_i} \) for each input image \( x_i \).


We assume that the attacker is fully informed about the vulnerabilities of each victim road sign but lacks knowledge of the specific sampling mask used in the defense algorithm.


\paragraph{Single Patch Attack}
The attacker possesses comprehensive knowledge of the defense mechanisms and employs a single patch attack aimed at exploiting known vulnerabilities. The goal is to find adversarial patch patterns such that:
\begin{align}
    y \neq f_{\alpha} (g_{\beta}(X+\delta))
\end{align}

This section addresses familiar attack types and should be completed swiftly due to familiarity with the method and adherence to the "don't think twice" policy. The types of attacks include:
\begin{enumerate}
    \item Patch Attack,
    \item Sticker Attack,
    \item Camouflage Attack—both derived from the study in \ref{}, concerning the vulnerability of stop signs.
\end{enumerate}

\paragraph{Proposed Multi Patch Attacks}
This attack strategy involves deploying multiple adversarial patches within the constraints of a given budget for attack size and number. This is a more complex attack because it allows the attacker to spawn multiple patches on the road signs, thereby increasing the likelihood of inducing misclassification.

\paragraph{Algorithm}
\textbf{Given:} Attack budget percent \( w \) and sub-patch size \( m \). 
\textbf{Return:} \( X_{\text{adv}} \)

\textbf{Step 1:} Classify patches into an informative patch set \( S_1 \) and a non-informative patch set \( S_2 \) based on their performance.

\textbf{Step 2:} For each \( \text{patch}_i \) in \( S_2 \):
\begin{itemize}
    \item Generate an adversarial patch on \( \text{patch}_i \),
    \item Decrement \( M \) by 1.
\end{itemize}
Repeat Step 2 until \( M = 0 \), indicating that the attack budget is exhausted.


==> attack_aware.tex <==
\subsection{Special Case: Attacker-Aware Robust Environmental Design (AA-RED)}
Next, we look at how RED can be improved when the defender has knowledge of the attacks, and designs specific robust signs for robustness against given attacks $A$; the set of attacks is $\delta$.
Let $\alpha$ be the robust pattern, it is label-specific, and each class has a robust pattern, let $f$ be the classification model, and let $L$ be the cross entropy loss:
% \textcolor{red}{AE: Check other papers and copy the way that they preset their equations (e.g. $\delta$). Also you should use \emph{underbrace} when defining things, e.g., $$F(x) = \underbrace{\sum_{x\in X} w_xf(x)}_{\text{weighted sum over the function $f$}}$$}
% \begin{align*}
% \min_{\alpha} \sum_i \left( \underbrace{ L(f(X'_{\alpha}), y_i)}_{\text{loss on clean images},\underbrace{ L(f(X_{\alpha}+\delta), y_i)}_{\text{loss on adv images} } \right)
% \end{align*}
\begin{align*}
f^*, \boldsymbol{\alpha} = \min_{\alpha, f} \max_{\delta} &\sum_i \left( \underbrace{L\big(f\big(g(X_{\alpha})\big), y_i\big)}_{\text{loss on clean images}} + \underbrace{L\big(f\big(g(X_{\alpha}+\delta)\big), y_i\big)}_{\text{loss on adv images}} \right)\\
&\text{ s.t. }~\delta~\text{ is defined by Equation \ref{eq:adv}}
\label{eq:AA_loss}
\end{align*}
That is when the attacker is known, the defender can simulate the attacker's best response $\delta$ to the defender's current choice of pattern $\boldsymbol{\alpha}$ and classifier $f$.
This is effectively a combination of adversarial training and RED. 
The full procedure for AA-RED is outlined in Algorithm \ref{alg:optimize_patterns_with_attack}



\begin{algorithm}
\caption{Attacker-Aware Robust Environmental Desing (AA-RED)}
\label{alg:optimize_patterns_with_attack}
\begin{algorithmic}[1]
\State \textbf{Input:} Dataset \(X, Y\) 
\State \textbf{Output:} Road sign backgrounds \(\boldsymbol{\alpha}\) for each class; \(\boldsymbol{\alpha} = \{\alpha_1, \cdots, \alpha_j, \ldots, \alpha_m \}\)
\State randomly initialize $\boldsymbol{\alpha}$
\For{each epoch}
    \State apply pattern $\alpha_y$ to each image $X$ with class $y$
    \State Generate ablated images using \(g\)
    \State Compute the attacker's best perturbation $\delta_i$ for each each modified image $X_{i, \alpha_{y_i}}$
    \State Compute the total loss $ \mathcal{L} = \sum_{i=1}^N \bigg(L\big(f\big(g(X_{i, \alpha})\big), y_i\big) 
 +L\big(f\big(g(X_{i, \alpha}+\delta)\big), y_i\big)\bigg)$
    \State Compute gradient of $\mathcal{L}$ w.r.t. to $\alpha$ and $f$, i.e. $\nabla_{\boldsymbol{\alpha}} L$ and $\nabla_{f} L$
    \State Update $\boldsymbol{\alpha}$ and $f$ according to $\nabla_{\boldsymbol{\alpha}}$ and $\nabla_{f}$
    % \If{epoch < 5}
    %     \State Update both \(f\) and \(\boldsymbol{\alpha}\) (warm-up phase)
    % \ElsIf{epoch \% 10 == 0}
    %     \State Update both \(f\) and \(\boldsymbol{\alpha}\)
    % \Else
    %     \State Update only \(\boldsymbol{\alpha}\)
    % \EndIf
\EndFor
\State \textbf{Return} \(\boldsymbol{\alpha}\), $f$
\end{algorithmic}
\end{algorithm}





==> conclusion.tex <==
\section{Conclusion}

This study introduces an environmental-centric approach to enhance the robustness of road sign recognition against adversarial attacks, proposing a new research direction to improve machine learning robustness by redesigning the physical world. 
To do this, we propose Robust Environmental Desing, an attacker agonist framework for modifying physical objects such that they are less susceptible to adversarial perturbations. 
Robust Environmental Design results in significant improvements in data separability and system generalization compared with model-centric approachs.
Robust Environmental Design can also be combined with these model-centric approaches (as we demonstrated with adversarial training).
These findings encourage the extension of robust design principles to broader applications to other computer vision domains, such as object detection and segmentation.
Future research should continue to refine these strategies under varied conditions to validate their effectiveness across different environments and threat models. The adoption of these robust design principles by industry stakeholders is crucial for advancing the safety and reliability of autonomous vehicles that rely on sign identification.
Although our focus is road sign classification, redesigning physical elements can be broadly applied in any setting for manufactured objects.
For example, one could extend our optimization framework to cars, clothing, buildings, etc.

% For instance, \cite{} demonstrates that adversarial examples, making several models in the self-driving pipeline vulnerable. 
% Examples include object detection \cite{}, segmentation \cite{}, and depth estimation \cite{}. Adversarial noise on a billboard \cite{} or patterns on the road \cite{} can cause an autonomous car to crash.
% Can redesigning car color schemes, road markings, and adding \emph{robust} watermarks make self-driving systems more robust?

==> no_aware_attack_backup.tex <==
\subsection{Robust Environmental Design (RED) }
% \textcolor{red}{This isnt a specific setting, this is your main method.}
\todo{Add the transition paragraph, or briefly discuss your method}

In this setting, the defender lacks specific knowledge of the attacker’s strategies, aware only that attacks appear as patches on road signs. 
The goal is to develop robust road signs that resist a wide array of patch-based attacks, regardless of patch shape or attack algorithms. Once deployed, these road signs should defend against adversarial patches using non-adversarial training-based defense algorithms.
\textcolor{red}{This paragraph is unlcear. You are trying to discuss to many thing in this paragraph. You should probably move some of them to the new Preliminaries section I created. Talking about the limitations of current road signs should go in preliminaries.}
We begin by introducing non-adversarial training-based defense algorithms designed to address patch attacks. 
This discussion encompasses an examination of the inherent limitations in the current designs of road signs when they are subjected to adversarial attacks, particularly highlighting the challenges when applying these specific defense algorithms. 
To overcome these limitations, we explore techniques for redesigning road sign patterns to ensure accurate predictions.

\textcolor{red}{Is this how autonomous vehicles work?}

This is how to train the road sign classification model. 
This should go to

% Autonomous vehicles perform road sign classification by initially capturing images of road signs from the environment. These images, comprising the dataset \(\mathbf{X}\), are then used to train a classification model \(f\) for road sign recognition.
% However, multiple studies \cite{} have demonstrated that these road sign classification models, denoted as \(f\) \textcolor{red}{You already defined f}, are vulnerable to malicious attacks. 
% Attackers can physically modify road signs by adding malicious patches, resulting in a modified road image \(X'\). \textcolor{red}{AE: This discussion about patch attacks needs to go in the preomilaries section, this section is about describing your method.} This malicious modification causes autonomous driving systems to perceive the changed image, leading the classification model $f$ to misclassify these modified signs, leading to incorrect predictions:
% \[
% f(X') \neq y,
% \]
% potentially resulting in severe safety hazards for autonomous vehicles.

Given the critical importance of safety in autonomous vehicles, our defensive strategy focuses on preemptive methods that are robust against adversarial attacks by design, rather than relying on post-attack remediation methods that typically require adversarial training.
The most commonly used preemptive defenses for patch attack is image ablation method. 
This method involves removing adversarial patches by randomly or strategically ablating parts of the modified image $X'$, forming a set of ablated images \( S' \). The set \( S' \) is then used for inference, aiming to ensure that \[ \underbrace{f(S')}_{\text{prediction for X' based on ablated images set}} = y, \] thus achieving correct predictions despite the presence of adversarial patches.

% To achieve this goal, the ablated images in \( S \) should predominantly be free of adversarial pixels \textcolor{red}{define adversarial pixles} as shown in \cite{reference}, while retaining discriminative information for accurate classification. 
% However, as \cite{reference} demonstrates, adversarial attackers often strategically place adversarial patches on crucial parts of the image, such as important areas of road signs, to impair inference. 
% Thus, if an ablated image successfully bypasses adversarial patches, it may also lose critical discriminative class information.
% Therefore, there is a fundamental trade-off between accuracy and the likelihood that an ablated image contains essential discriminative information.
% To address this tradeoff, prior works \cite{reference} focus on developing strategic ablation algorithms. 
% However, no method has yet achieved high accuracy in road sign classification applications. 
% One major reason is that the set \( S \) often loses crucial inference information.

\textcolor{red}{This paragraph should be in the next section. You want to just have one section where you propose your idea.}
Therefore, we propose an orthogonal research direction, we propose to achieve the performance of \( f(S) \) by redesigning the appearance of \( X \), such as the background of road signs. 
% \underbrace{\sum_{x\in X} w_xf(x)}_{\text{weighted sum over the function $f$}}$$}
Let \( \alpha \) represent the pattern of the road sign background, and \( X_{\alpha} \) be the redesigned image with the \( \alpha \) background. To achieve robust predictions, we aim to find \( \alpha \) such that
$$\underbrace{f(s_i)}_{\text{prediction of $i^{th}$ ablated image}} = y, \forall s_i \in S_{\alpha}$$

where \( S_{\alpha} \) is the set of ablated images derived from \( X_{\alpha} \).
% Note that our method can be combined with any image ablation method.

\paragraph{Robust Road Sign Design} \textcolor{red}{Way too technical for a deep learning paper. You should give a plain English description, then mention the specifics. The last paragraph from the previous section would be particularly helpful for this. You haven't actually described what your objective is. Why should I care about some abletion algorithm $g$ or a dataset???????} Given an image ablation algorithm $g$,  a dataset \((X, Y)\), where \(X = \{x_1, x_2, \ldots, x_n\}\) contains images and \(Y = \{y_1, y_2, \ldots, y_n\}\) are the corresponding labels with \(m\) unique labels, our goal is to minimize the cross-entropy loss for ablated images derived from each image in \(X\). Each image \(x_i\) is processed by an image ablation algorithm $g$, producing a set of ablated images \(S_i\). The objective function can be formulated as follows:

\begin{equation}
\label{eq:min_alpha}
\min_{\alpha} \sum_{i=1}^n \sum_{s \in S_i(\alpha)} \underbrace{L(f(s), y_i)}_{\text{cross entropy loss between the prediction of an ablated image and its label}}
\end{equation}

where \(S_i(\alpha)\) represents the set of ablated images derived from \(X_i\) using the given ablation algorithm $g$, \(f(s; \alpha)\) denotes the prediction model output for ablated image \(s\), which is also influenced by \(\alpha\), and \(L\) is the cross-entropy loss function that compares the predicted label \(f(s; \alpha)\) against the true label \(y_i\).
This objective function is designed to optimize \(\boldsymbol{\alpha}\) by improving classification accuracy across a diversely ablated dataset, thus enhancing the model's robustness to variations and imperfections in image data.

We utilize gradient-based optimization for \(\alpha\) as outlined in Algorithm \ref{alg:train}. 
The procedure initiates with several warm-up epochs to train the model while updating robust design parameters $\alpha$. 
Including the training of the model in the warm up is to providing essential directional guidance for $\alpha$ to adjust. 
Subsequently, the training focus the updating the robust parameters $\alpha$, the model parameters will only updated every few epochs based on new insights gained from the ongoing training process.
\begin{algorithm}
\caption{Training Algorithm}
\label{alg:train}
\begin{algorithmic}[1]
\State \textbf{Input:} Dataset \(X, Y\), ablation algorithm \(g\).
\State \textbf{Output:} Trained robust road sign backgrounds \(\boldsymbol{\alpha}\) for each class; \(\boldsymbol{\alpha} = \{\alpha_1, \cdots, \alpha_j, \ldots \alpha_m \}\)

\State Initialize \(\alpha_j\) for each road sign class \(j\); 


\For{epoch in num\_epochs}
    \State Get the set of ablated images via $g$.
    \State \(l = \sum_{i=1} \sum_{x\in S_i(\alpha)} L(f(s),y_i)\)
    \State \(l.backward()\)
    \If{epoch < 5}
        \State Update \(f\) and \(\boldsymbol{\alpha}\) (warm-up phase)
    \ElsIf{epoch \% 10 == 0}
        \State Update \(f\) and \(\boldsymbol{\alpha}\)
    \Else
        \State Update only \(\boldsymbol{\alpha}\)
    \EndIf
\EndFor
\State \textbf{Return} \(\boldsymbol{\alpha}\)
\end{algorithmic}
\end{algorithm}

\paragraph{Image Ablation}
In the next analysis, we address two pivotal questions that significantly impact the image ablation defense: \emph{How to ablate image x to get \(S\)?} and \emph{How to use \(S\) for inference?}

For an ablated image $s_i$, the area of the reserved image should be small to avoid the including adversarial pixel. This is crucial for defending against patch attack.  
This is because adversarial patch attacks are often characterized as \( \ell_\infty \) attacks, which allow attackers to modify the pixels within patches arbitrarily. 
This type of attack typically results in patches that deviate significantly from the distribution of clean, unaltered patches, thereby diminishing the effectiveness of traditional models that have not been trained adversarially. 

More specifically, if a patch \( z \) contains adversarial pixels, it is highly probable that the model's prediction \( f(z) \) will not correspond to the true label \( y \). 
Given this scenario, the area of the reserved image in s used for inference is crucial. Using s that reserve small area can mitigate the impact of adversarial modifications by decreasing the likelihood that s will contain adversarial pixels, thereby enhancing the effectiveness of the defense.
\ref{} theoretically discusses and confirms the probability of avoiding adversarial pixels is highly related to the reserved area in s.

Given an ablated image \( s \) that removes the majority of the original image, if it does not contain adversarial information, the subsequent question is whether it still retains sufficient class information to ensure that \( f(s) = y \).


\paragraph{Enhance Class Information within a Road Sign}

We then explore whether the class of a road sign can be accurately determined from only a small visible area. \textcolor{red}{You are now talking about something experimental. This does not go in a preliminaries section. Describe your method, that's it. We don't "explore" things in prelimnaries or methodology sections. If something is important to your method, such as the small visible area, then just say "in practice we observe that smaller patches regions are more effective (see Section \ref{} for more a more through study of region size.} Our findings across both the LISA and GTSRB datasets reveal that current sign designs typically require a relatively large visible area for effective inference. To address this issue, we propose redesigning road signs to enhance the informational content within small local area, say small patches. 

Without loss of generality, we consider an ablation algorithm \( g \), detailed in Algorithm \ref{alg_label}, which obscures most of the image while retaining only a small patch. 
Consequently, an ablated sample \( s \) will contain just this small patch of the original image \( X \).
This approach serves as a showcase for the robust road sign design. 

We employ Algorithm \ref{alg:train} to optimize the design of robust road sign backgrounds. These backgrounds are engineered to enhance the class information within localized small areas. Consequently, as illustrated in Figure \ref{fig:road_sign_design}, every local area of the newly designed road signs contains essential class information.
This redesigned strategy aims to ensure that even minimal patches can independently verify the sign's class, i.e., \( f(s) = y \), thereby enhancing accuracy and robustness.

We address the selection of patch sets \( S \) for inference, where \cite{} suggests using a random patch. We expand on this by employing algorithm \cite{} to cover the image fully and use a majority vote for prediction. While single random patch sampling provides some resistance, it remains susceptible to attacks unless most patches are compromised. In contrast, the majority vote approach only fails if over half the patches are adversarially altered. This method proves particularly effective for road signs, maintaining robustness unless more than 50\% of the patches are misleadingly modified. Both methods are evaluated in our experiments.

\textcolor{red}{These aglorihms are good, but can you also give a plain English version. Don't get ride of these algorithms, but give a second version that is more plain english.}
\begin{algorithm}
\caption{Ablated Images Set Collection}
\label{alg:ablated_images}
\begin{algorithmic}[1]
\State \textbf{Input:} Image $X'$, patch size $a$, classification model $f$.
\State \textbf{Output:} Set of ablated images $S$.
\State Initialize $S = []$, $W, H = \text{dimensions of } X'$ 
\For{$i = 0$ to $\frac{W}{a} - 1$}
    \For{$j = 0$ to $\frac{H}{a} - 1$}
        \State Create mask with ones at $[i \cdot a:(i+1) \cdot a, j \cdot a:(j+1) \cdot a]$ and zeros elsewhere
        \State $s = \text{mask} \times X'$  % Element-wise multiplication
        \State Append $s$ to $S$
    \EndFor
\EndFor
\State \textbf{Return} $S$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Majority Vote Inference Algorithm}
\label{alg:majority_vote}
\begin{algorithmic}[1]
\State \textbf{Input:} Image $X'$, mask size $a$, model $f$.
\State \textbf{Output:} Prediction for $X'$.
\State $S \leftarrow$ Set of ablated images from Algorithm \ref{alg:ablated_images}.
\State Initialize $P = []$.
\For{each $s$ in $S$}
    \State $P \leftarrow P \cup \{f(s)\}$  % Append model prediction for each patch
\EndFor
\State $y_p \leftarrow \text{majority\_vote}(P)$  % Compute majority vote from predictions
\State \textbf{Return} $y_p$
\end{algorithmic}
\end{algorithm}







==> relate_work_prior.tex <==



% ##################################
% ##################################

% IBCD is a two-stage defense method that estimates patch size and applies certified defenses to counter adversarial patch attacks, enhancing robustness in real-world black-box scenarios without prior knowledge of patch position or size.

% 6. Architecture-Agnostic Iterative Black-Box Certified Defense Against Adversarial Patches

##################################
##################################
PatchCensor \cite{10.1145/3591870} certifies the patch robustness of Vision Transformers (ViT) by using exhaustive testing and voting over multiple inferences with different attention masks. It provides high certified accuracy against worst-case patch attacks with minimal impact on clean accuracy, outperforming state-of-the-art methods.

7. Patchcensor: Patch robustness certification for transformers via exhaustive testing

@article{10.1145/3591870,
author = {Huang, Yuheng and Ma, Lei and Li, Yuanchun},
title = {PatchCensor: Patch Robustness Certification for Transformers via Exhaustive Testing},
year = {2023},
issue_date = {November 2023},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {32},
number = {6},
issn = {1049-331X},
url = {https://doi.org/10.1145/3591870},
doi = {10.1145/3591870},
abstract = {In the past few years, Transformer has been widely adopted in many domains and applications because of its impressive performance. Vision Transformer (ViT), a successful and well-known variant, attracts considerable attention from both industry and academia thanks to its record-breaking performance in various vision tasks. However, ViT is also highly nonlinear like other classical neural networks and could be easily fooled by both natural and adversarial perturbations. This limitation could pose a threat to the deployment of ViT in the real industrial environment, especially in safety-critical scenarios. How to improve the robustness of ViT is thus an urgent issue that needs to be addressed. Among all kinds of robustness, patch robustness is defined as giving a reliable output when a random patch in the input domain is perturbed. The perturbation could be natural corruption, such as part of the camera lens being blurred. It could also be a distribution shift, such as an object that does not exist in the training data suddenly appearing in the camera. And in the worst case, there could be a malicious adversarial patch attack that aims to fool the prediction of a machine learning model by arbitrarily modifying pixels within a restricted region of an input image. This kind of attack is also called physical attack, as it is believed to be more real than digital attack. Although there has been some work on patch robustness improvement of Convolutional Neural Network, related studies on its counterpart ViT are still at an early stage as ViT is usually much more complex with far more parameters. It is harder to assess and improve its robustness, not to mention to provide a provable guarantee. In this work, we propose PatchCensor, aiming to certify the patch robustness of ViT by applying exhaustive testing. We try to provide a provable guarantee by considering the worst patch attack scenarios. Unlike empirical defenses against adversarial patches that may be adaptively breached, certified robust approaches can provide a certified accuracy against arbitrary attacks under certain conditions. However, existing robustness certifications are mostly based on robust training, which often requires substantial training efforts and the sacrifice of model performance on normal samples. To bridge the gap, PatchCensor seeks to improve the robustness of the whole system by detecting abnormal inputs instead of training a robust model and asking it to give reliable results for every input, which may inevitably compromise accuracy. Specifically, each input is tested by voting over multiple inferences with different mutated attention masks, where at least one inference is guaranteed to exclude the abnormal patch. This can be seen as complete-coverage testing, which could provide a statistical guarantee on inference at the test time. Our comprehensive evaluation demonstrates that PatchCensor is able to achieve high certified accuracy (e.g.,&nbsp;67.1\% on ImageNet for 2\%-pixel adversarial patches), significantly outperforming state-of-the-art techniques while achieving similar clean accuracy (81.8\% on ImageNet). The clean accuracy is the same as vanilla ViT models. Meanwhile, our technique also supports flexible configurations to handle different adversarial patch sizes by simply changing the masking strategy.},
journal = {ACM Trans. Softw. Eng. Methodol.},
month = {sep},
articleno = {154},
numpages = {34},
keywords = {Adversarial patch, neural networks, robustness certification, vision transformer, certified accuracy, deep learning}
}

##################################
##################################

\cite{10.1145/3579856.3582816} Jujutsu detects and mitigates adversarial patch attacks on DNNs by identifying influential localized features and using GANs to reconstruct clean inputs. It outperforms existing defenses across multiple datasets and models, effectively handling physical-world and adaptive attacks.

8. Jujutsu: A two-stage defense against adversarial patch attacks on deep neural networks
@inproceedings{10.1145/3579856.3582816,
author = {Chen, Zitao and Dash, Pritam and Pattabiraman, Karthik},
title = {Jujutsu: A Two-stage Defense against Adversarial Patch Attacks on Deep Neural Networks},
year = {2023},
isbn = {9798400700989},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3579856.3582816},
doi = {10.1145/3579856.3582816},
abstract = {Adversarial patch attacks create adversarial examples by injecting arbitrary distortions within a bounded region of the input to fool deep neural networks (DNNs). These attacks are robust (i.e., physically-realizable) and universally malicious, and hence represent a severe security threat to real-world DNN-based systems. We propose Jujutsu, a two-stage technique to detect and mitigate robust and universal adversarial patch attacks. We first observe that adversarial patches are crafted as localized features that yield large influence on the prediction output, and continue to dominate the prediction on any input. Jujutsu leverages this observation for accurate attack detection with low false positives. Patch attacks corrupt only a localized region of the input, while the majority of the input remains unperturbed. Therefore, Jujutsu leverages generative adversarial networks (GAN) to perform localized attack recovery by synthesizing the semantic contents of the input that are corrupted by the attacks, and reconstructs a “clean” input for correct prediction. We evaluate Jujutsu on four diverse datasets spanning 8 different DNN models, and find that it achieves superior performance and significantly outperforms four existing defenses. We further evaluate Jujutsu against physical-world attacks, as well as adaptive attacks.},
booktitle = {Proceedings of the 2023 ACM Asia Conference on Computer and Communications Security},
pages = {689–703},
numpages = {15},
keywords = {Adversarial robustness, Deep learning, Neural networks, Security},
location = {<conf-loc>, <city>Melbourne</city>, <state>VIC</state>, <country>Australia</country>, </conf-loc>},
series = {ASIA CCS '23}
}
##################################
##################################
Feature Partition Aggregation (FPA) is a certified defense against L0 evasion, backdoor, and poisoning attacks. It uses an ensemble of submodels trained on disjoint feature sets, providing stronger and faster robustness guarantees than current L0 defenses.

##################################
##################################

PatchCleanser \cite{xiang2021patchcleanser} defends against adversarial patch attacks by using two rounds of pixel masking to neutralize adversarial effects, ensuring compatibility with state-of-the-art classifiers.

11. Proceedings of the IEEE/CVF International Conference on
Computer Vision, pages 4842–4851, 2019.
Certifiably robust defense against adversarial patches for any image classifier.




##################################
##################################

1. Advances in adversarial attacks and defenses in computer vision: A survey
2. Interpreting adversarial examples in deep learning: A review
4. Adversarial attacks and robust defenses in deep learning






==> related_work.tex <==
\section{Related Work}

\paragraph{Road Sign Classification Attack}
Adversarial attacks on road sign recognition systems are critical due to their safety implications for autonomous driving. Goodfellow et al. \cite{goodfellow2014explaining} highlighted the vulnerability of neural networks to adversarial examples. Madry et al. \cite{madry2017towards} demonstrated the practical dangers of these examples, particularly in autonomous vehicles where misclassification can lead to severe accidents.

Adversarial patches, which alter a small region of an image to deceive classifiers, have been extensively studied. Brown et al. \cite{brown2017adversarial} introduced physical adversarial patches for real-world objects, including road signs. Eykholt et al. \cite{eykholt2018robust} showed that adversarial stickers could cause misclassification, emphasizing the need for robust defenses. Following this, \cite{liu2018delving}, \cite{karmon2018lavan}, and \cite{zhang2019robust} applied patch attacks to other image recognition tasks.

\paragraph{Defending Against Adversarial Patch Attacks}
Various techniques address classifier vulnerabilities to patch-based attacks, categorized into:

\paragraph{Attack-Aware Defenses} These require knowledge of specific attacks or attacker types. Adversarial training augments training data with adversarial examples to improve robustness \cite{goodfellow2014explaining,shafahi2019adversarial,madry2017towards, ilyas2019adversarial, tsipras2018robustness, ross2018improving, carlini2017towards,wong2018provable, tramer2017ensemble, athalye2018obfuscated}. PatchGuard \cite{xiang2020patchguard} and PatchCleanser \cite{xiang2022patchcleanser} use small receptive fields and masking to identify patch locations, requiring prior knowledge of attack patch size.

\paragraph{Attack-Agnostic Defenses} These do not require specific attack knowledge. Randomized smoothing enhances robustness by adding random noise to input data at test time \cite{cohen2019certified, lecuyer2019certified, li2018second, salman2019provably, jeong2020consistency, zhang2020certifying}.

Defending against adversarial patches often involves sanitizing the patch via ablation algorithms. Efforts to develop certifiably robust defenses include works by \cite{xiang2020patchguard, chiang2020certified, levine2020randomized, metzen2021efficient, xiang2021patchguard, xu2023patchzero, zhang2020clipped, chattopadhyay2023defensivedr}, with PatchGuard \cite{xiang2020patchguard} using small receptive fields and outlier masking.

% \bibliographystyle{plain}
% \bibliography{references}


% \section{Related Work}
% Adversarial attacks on road sign recognition systems have become a critical area of research due to their potential safety implications for autonomous driving. Goodfellow et al. \cite{goodfellow2014explaining} were among the first to highlight the vulnerability of deep neural networks to adversarial examples. Madry et al. \cite{madry2017towards} further explored this by demonstrating that adversarial examples can be crafted to fool robust models in practical scenarios. These attacks have been shown to be particularly dangerous in the context of autonomous vehicles, where a misclassification of road signs can lead to severe accidents. The concept of adversarial patches, which involves altering a small region of an image to fool the classifier, has been extensively studied. Brown et al. \cite{brown2017adversarial} introduced adversarial patches that can be physically applied to real-world objects, including road signs, to deceive classifiers. Subsequent research by Eykholt et al. \cite{eykholt2018robust} demonstrated that strategically placed adversarial stickers can cause misclassification of road signs, highlighting the need for robust defense mechanisms. 
% Follow by this work, \cite{liu2018delving,karmon2018lavan,zhang2019robust} use patch attack for physically attacking patch attack for other image recongnition tasks. 

% To defend against patch attacks.
% Various model-centric techniques have been proposed to address the vulnerability of classifiers to patch-based attacks. These techniques can be roughly categorized into two sets: 1) Attack-Aware Defenses, such as the methodoglies that involves adversarial training (To strengthen vital computer vision systems, concerted efforts have been made to develop certifiably robust defenses against adversarial patches \cite{chiang2020certified,levine2020randomized,metzen2021efficient,xiang2021patchguard,zhang2020clipped}. These defense strategies aim to provide a certifiable guarantee for making accurate predictions on select images. In this vein, \cite{xiang2020patchguard} pioneered the use of PatchGuard, a network that utilizes a small receptive field and outlier masking. Building on this, \cite{xiang2022patchcleanser} proposed a defense mechanism that leverages an ensemble and an exhaustive masking technique to identify the location of the patch. It's important to note that both methods require prior knowledge of the size of the attack patch. )
% Adversarial training is a technique used to improve the robustness of neural networks against adversarial attacks. It involves augmenting the training data with adversarial examples to help the model learn to resist such attacks. 
% \cite{goodfellow2014explaining, shafahi2019adversarial, madry2017towards, ilyas2019adversarial, tsipras2018robustness, ross2018improving, carlini2017towards, wong2018provable, tramer2017ensemble, athalye2018obfuscated,shafahi2019adversarial, tramer2017ensemble}

% The o
% and 2) Attack-Agnostic Defenses don't  require knowledge of specific attacks to build effective countermeasures. For example, randomized smoothing, which a technique used to enhance the robustness of neural networks against adversarial attacks by adding random noise to the input data at test time. Several have demonstrated the effectiveness of randomized smoothing in defending against adversarial examples \cite{cohen2019certified, lecuyer2019certified, li2018second, salman2019provably, jeong2020consistency, zhang2020certifying, chiang2020detection, feng2020noise, horvath2021boosting, kim2021bridging}.

% In particalur, to defend agaisnt adversarial patches,
% sanitizing the adverarial patch by ablation algorithm , 
% To strengthen vital computer vision systems, concerted efforts have been made to develop certifiably robust defenses against adversarial patches \cite{xiang2020patchguard, chiang2020certified,levine2020randomized,metzen2021efficient,xiang2021patchguard,xu2023patchzero,zhang2020clipped,hattopadhyay2023defensivedr}. These defense strategies aim to provide a certifiable guarantee for making accurate predictions on select images. In this vein, \cite{xiang2020patchguard} pioneered the use of PatchGuard, a network that utilizes a small receptive field and outlier masking. 




==> training.tex <==
\paragraph{Training Pipeline}
The primary goal of our project is to deploy redesigned road signs into the physical world. These signs are then captured by cameras, serving as inputs for the road sign classification systems in autonomous driving models.

\textbf{Challenges and Solutions:}
Direct experimentation in the physical world to determine optimal sign colors is infeasible due to high costs, logistical complexities, and the non-differentiable nature of the physical testing process. These challenges prevent the direct application of gradient-based optimization methods for parameter updates. Therefore, we propose a differentiable approximation training pipeline to effectively find the optimal parameters.

\textbf{Pre-training Setup:}
Before training begins, camera calibration ensures accurate color representation and spatial alignment for consistency in various environmental conditions. We utilize a simulated environment that mirrors the physical conditions affecting road signs, involving:
- \(C\): serval neural networks for color mapping from designed signs to camera-captured images.
- \(H\): A 3x3 homography matrix for spatial adjustments due to camera angles and sign placement.
Color mappings are determined by sampling and photographing color patches in real-world settings.
The training pipeline and its components are illustrated in Figure \ref{}, which details the flow from sign design to image capture and processing within the autonomous driving model.

\paragraph{Training Algorithm and Objective Function}
To bolster model \(f\) robustness against adversarial attacks, our training involves iterative adversarial perturbation generation and model updates:
\begin{enumerate}
    \item \textbf{Adversarial Perturbation Generation:} Each iteration \(i\) utilizes model parameters \(f_i\) and robustness parameter \(\alpha_i\) to identify the adversarial perturbation \(\delta_i\) that maximizes cross-entropy loss:
    \[
    \delta_i = \arg\max_{\delta} L(f_i(g(X + \delta, \alpha_i)), y)
    \]
    where \(g\) is the preprocessing applied to \(X\) and \(y\) is \(X\)'s true label. Off-the-shelf methods are available for generating \(\delta\).
    \item \textbf{Model and Robustness Parameter Update:} "Robustness parameter" refers to model settings that enhance its defense. Update \(f\) and \(\alpha\) at iteration \(i+1\) to minimize the loss with the adversarial perturbation \(\delta_i\):
    \[
    f_{i+1}, \alpha_{i+1} = \arg\min_{f, \alpha} L(f(g(X + \delta_i, \alpha)), y)
    \]
\end{enumerate}
This process alternates between maximizing adversarial effects using \(\delta\) and reducing impacts via updates to \(f\) and \(\alpha\), enhancing resistance to future attacks.



\todo{Add a distribution figure for showing how the distribution comparison for clean examples and  adversarial examples, current design vs. robust design, is affected.}

One intuition behind robust design is that by increasing the dimensions of the input space, data points become more separable after adversarial training, enhancing the system's ability to generalize and resist adversarial attacks. This can be achieved through techniques like feature engineering or using higher-dimensional representations of the input data.



\subsection{Training}
\paragraph{Image Compositing Pipeline}

spatial and color mappings. 



\begin{algorithm}
\textbf{Training Algorithm:}
\begin{algorithmic}[1]
\For{$i$ in range(epochs)}
    \State Sample $M$ patches from the image $X$: $S = g(X)$
    \For{$j$ in range($M$)}
        \State Train $f(S_j)$
    \EndFor
\EndFor
\State \textbf{Return} $f$
\end{algorithmic}
\end{algorithm}
